Dynamic data structures for parameterized string problems

We revisit classic string problems considered in the area of parameterized complexity, and study them through the lens of dynamic data structures. That is, instead of asking for a static algorithm that solves the given instance efficiently, our goal is to design a data structure that efficiently maintains a solution, or reports a lack thereof, upon updates in the instance. We first consider the Closest String problem, for which we design randomized dynamic data structures with amortized update times $d^{\mathcal{O}(d)}$ and $|\Sigma|^{\mathcal{O}(d)}$, respectively, where $\Sigma$ is the alphabet and $d$ is the assumed bound on the maximum distance. These are obtained by combining known static approaches to Closest String with color-coding. Next, we note that from a result of Frandsen et al.~[J. ACM'97] one can easily infer a meta-theorem that provides dynamic data structures for parameterized string problems with worst-case update time of the form $\mathcal{O}(\log \log n)$, where $k$ is the parameter in question and $n$ is the length of the string. We showcase the utility of this meta-theorem by giving such data structures for problems Disjoint Factors and Edit Distance. We also give explicit data structures for these problems, with worst-case update times $\mathcal{O}(k2^{k}\log \log n)$ and $\mathcal{O}(k^2\log \log n)$, respectively. Finally, we discuss how a lower bound methodology introduced by Amarilli et al.~[ICALP'21] can be used to show that obtaining update time $\mathcal{O}(f(k))$ for Disjoint Factors and Edit Distance is unlikely already for a constant value of the parameter $k$.

==> chapters/conclusion.tex <==
\section{Conclusion}




==> chapters/edit-distance.tex <==
\section{Edit Distance}

There is common dynamic algorithm to count edit distance:
$$ d_{i,j}  = 
    \begin{cases}
    
        j & \text{for $i = 0$}\\
        i & \text{for $j = 0$}\\
        d_{i-1, j-1} & \text{for $X[i] = Y[j]$}\\
        1 + min
        \begin{cases}
              d_{i-1, j}\\
              d_{i, j-1}\\
              d_{i-1, j-1}\\
        \end{cases} & \text{for $X[i] \neq Y[j]$}\\
    \end{cases}  $$
    where $ED(X,Y) = d_{|X|,|Y|}$.


% First we will show our result for Longest Common Subsequent - subproblem for Edit Distance where $w_{del}$, $w_{ins}$, and $w_{sub}$ are constant functions equal $1$.

% \subsubsection{Longest Common Subsequent}
% \mateusz{Levenshtein ref}
    

Let $suf_i$ denote the suffix $S_{i..n}$ of string $S$. The longest common extension of $X$ and $Y$ for $(i, j)$ is the longest prefix of suffixes $suf_i$ and $suf_j$. Let $LCE(i,j)$ be a longest common extension function, in other words: 
$$X[i + LCE(i,j) + 1] \neq Y[j + LCE(i,j) + 1] \land \forall_{d=0}^{LCE(i,j)}X[i+d] = Y[i+d]$$

Dynamic $d$ has $|X|*|Y|$ states that they need to be counted. Our idea is to use $LCE(i,j)$ to decrease this number.

% \subsubsection{Improve number of consider states}

\begin{lemma}
    Let $l = LCE(i,j)$. If we consider state $d_{i,j}$ we could instead consider state $d_{i + l, j+l}$.
\end{lemma}
\begin{proof}
    \mateusz{from paper. Czy jakoś bardziej jakos tłumaczymy to. Mogę dodać obrazek} 
\end{proof}

\begin{lemma}
    We can visit at most $3^e$ states of dynamic $d_{i,j}$ to count $d_{|X|, |Y|}$, where $e = ED(|X|,|Y|)$. 
\end{lemma}
\begin{proof}
    Our idea is to use $BFS$ to compute path from $d_{0,0}$ to $d_{|X|, |Y|}$. 
    We will only consider states $d_{i,j}$ that $LCE(i,j)=0$. If we are in the state $d_{i,j}$ there is three possible moves from this state to state one further:
    \begin{itemize}
        \item $d_{i + 1 + k_1,j + k_1}$ where $k_1 = LCE(i+1, j)$
        \item $d_{i + 1 + k_2,j + 1 + k_2}$ where $k_2 = LCE(i+1, j + 1)$
        \item $d_{i + k_3,j + k_3}$ where $k_3 = LCE(i, j + 1)$
    \end{itemize}
    From every state we could go 3 other states and there is a path that use $e$ states, so the number of considered states are $O(3^e)$.
\end{proof}


\begin{lemma}
    We can visit at most $O(e^2)$ states of dynamic $d_{i,j}$ to count $d_{|X|, |Y|}$. 
\end{lemma}
\begin{proof}
    This is similar idea like in previous Lemma's proof, but with extra observation. If we consider two states $d_{i,j}$ and $d_{i + x,j + x} \land x>0$ with the same distance, then every move from $d_{i+x,j+x}$ leads to the same state or further, so we don't need to analyze $d_{i,j}$.
    
    Let $b$ be current consider distance in $BFS$ algorithm. Let $diag[b][t] \land -b \leq t \leq b$ be a dynamic such that $x = diag[b][t]$ means that there is a path of length $b$ from $d_{0,0}$ to $d_{x + t, x}$ and there is no such $x<y$ that $d_{y + t, y}$ is achievable in distance $b$.
    
    The formula for this dynamic:
    
    $$
    diag[b+1][t] = LCE(x+t, x) \text{, where}$$
    
    $$
    x = max \begin{cases}
            diag[b][t+1] + 2 \\
            diag[b][t] + 1 \\
            diag[b][t-1] \\
        \end{cases}
        $$

    Therefore $d_{|X|,|Y|} = diag[e][|X|-|Y|]$ and size of $diag$ is $O(e^2)$.
\mateusz{Nie jest to najładniejszy dowód, ale również Michał miał inny pomysł na niego. Mogę go poprawić, albo przypomnieć sobie Michała. Nie wiem czy traktować czytających jak gumową kaczuszkę czy zostawić więcej jako "łatwo widać, że". Mogę nawet dodać obrazek jbc.}

\end{proof}

\begin{corollary} \label{ed:corollary}
    Edit Distance for $X,Y \in \Sigma^{\star}$ can be computed in time $O(e^2 * LCE_{query} + LCE_{init} )$ where $LCE_{query}/LCE_{init}$ is time complexity for query/init. 
\end{corollary}

\begin{lemma}
    Static Edit Distance can be computed in $O(e^2 + n)$.
\end{lemma}
\begin{proof}
    $LCE$ can be computed by using suffix tree, so $LCE_{init}$ is in $O(n)$ and $LCE_{query}$ is in $O(1)$.
    \mateusz{Czy chcemy sie bardziej rozpisać}.
\end{proof}

\begin{corollary}
     Static $k$-Edit Distance can be computed in $O(k^2 + n)$.
\end{corollary}

% \subsubsection{Dynamic $k$-Longest Common Extension}


\defproblem{Dynamic $k$-Longest Common Extension}{Maintain a words $X, Y \in \Sigma^{\star}$}{
Maintain a function $LCE(i,j)$ such that $|i-j| \leq k \land X[i + LCE(i,j) + 1] \neq Y[j + LCE(i,j) + 1] \land \forall_{d=0}^{LCE(i,j)}X[i+d] = Y[i+d]$.}

\begin{lemma} \label{ed:lce}
    One can maintain words $X,Y \in \Sigma^{\star}$ and answer opertaions: 
    \begin{itemize}[noitemsep, topsep=0pt]
        \item $LCE_{update}(word, position, new letter)$ in $O(k \log \log n)$
        \item $LCE_{query}(i,j)$ in $O(\log \log n)$
        \item  $LCE_{init}(X,Y,k)$ in $O(kn)$
    \end{itemize}
\end{lemma}

\begin{proof}
    We will maintain for every diagonal $t \in [-k\dots k]$ one structure $s[t]$ to solve \textit{Interval Union-Split-Find}.
    \begin{algorithm}
        \SetKwFunction{Fupdate}{$LCE_{update}$}
        \SetKwProg{Fn}{Function}{:}{}
            \Fn{\Fupdate{$X$, $position$, $letter$}}{
             \tcc{There is a similar function for changing $Y$, but little more complicated}
              \For{$t \in [-k \dots k] $}{
                 \uIf{$X[i + t] == letter$}{
                    s[t].unmark(position) \;
                    }   
                 \Else {
                   s[t].mark(position) \;
                   }
                }
                Y[position] = $letter$ \;
            }
            
      \SetKwFunction{Fquery}{$LCE_{query}$}
            \Fn{\Fquery{$i$, $j$}}{
               \KwRet s[i - j].find(i)\;
            }
    
    \end{algorithm}
\mateusz{Zmienic na Van Emde Boasa (zrobiłem na podstawie k-disjoint factors)}
\end{proof}

\begin{lemma}
    One can maintain words $X,Y \in \Sigma^{\star}$ and answer opertaions: 
    \begin{itemize}[noitemsep, topsep=0pt]
        \item $ED_{update}(word, position, letter)$ in $O(k \log \log n)$
        \item $ED_{query}()$ in $O(k^2 \log \log n)$
        \item  $ED_{init}(X,Y,k)$ in $O(kn)$
    \end{itemize}
\end{lemma}

\begin{proof}
    It is a combination of Corollary \ref{ed:corollary} and Lemma \ref{ed:lce}
\end{proof}


==> chapters/related_work.tex <==
\section{Related Work}

